Configuring Cloud-Service Interfaces Using Flow Inheritance

Technologies for composition of loosely-coupled web services in a modular and flexible way are in high demand today. On the one hand, the services must be flexible enough to be reused in a variety of contexts. On the other hand, they must be specific enough so that their composition may be provably consistent. The existing technologies (WS-CDL, WSCI and session types) require a behavioural contract associated with each service, which is impossible to derive automatically. Furthermore, neither technology supports flow inheritance: a mechanism that automatically and transparently propagates data through service pipelines. This paper presents a novel mechanism for automatic interface configuration of such services. Instead of checking consistency of the behavioural contracts, our approach focuses solely on that of data formats in the presence of subtyping, polymorphism and flow inheritance. The paper presents a toolchain that automatically derives service interfaces from the code and performs interface configuration taking non-local constraints into account. Although the configuration mechanism is global, the services are compiled separately. As a result, the mechanism does not raise source security issues despite global service availability in adaptable form.

==> eptcsdata.tex <==
\providecommand{\firstpage}{27}
\providecommand{\publicationstatus}{R. Behjati and A. Elmokashfi (Eds.): Workshop on\\
Formal Methods for and on the Cloud (iFMCloud'16)\\
EPTCS 228, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.228.4}{10.4204/EPTCS.228.4}}
\pdfoutput=1

